ActivityEditor: Learning to Synthesize Physically Valid Human Mobility

Human mobility modeling is indispensable for diverse urban applications. However, existing data-driven methods often suffer from data scarcity, limiting their applicability in regions where historical trajectories are unavailable or restricted. To bridge this gap, we propose \textbf{ActivityEditor}, a novel dual-LLM-agent framework designed for zero-shot cross-regional trajectory generation. Our framework decomposes the complex synthesis task into two collaborative stages. Specifically, an intention-based agent, which leverages demographic-driven priors to generate structured human intentions and coarse activity chains to ensure high-level socio-semantic coherence. These outputs are then refined by editor agent to obtain mobility trajectories through iteratively revisions that enforces human mobility law. This capability is acquired through reinforcement learning with multiple rewards grounded in real-world physical constraints, allowing the agent to internalize mobility regularities and ensure high-fidelity trajectory generation. Extensive experiments demonstrate that \textbf{ActivityEditor} achieves superior zero-shot performance when transferred across diverse urban contexts. It maintains high statistical fidelity and physical validity, providing a robust and highly generalizable solution for mobility simulation in data-scarce scenarios. Our code is available at: https://anonymous.4open.science/r/ActivityEditor-066B.

==> latex/table/dataset.tex <==
\begin{table}[ht]
\centering
\small
\begin{tabular}{lrc}
\toprule
\textbf{Dataset} & \textbf{Sample Size (HH)} & \textbf{Scope} \\
\midrule
2017 NHTS & 129,603 & National (US) \\
California HTS & 42,500 & State (CA) \\
Mexico City OD Survey & 66,625 & Metro (MX) \\
Puget Sound Study & 3,285 & Regional (WA) \\
\bottomrule
\end{tabular}
\caption{Summary of HTS datasets used for model training and transferability evaluation. (HH: Households)}
\label{tab:dataset_stats}
\end{table}
